TTSOps: A Closed-Loop Corpus Optimization Framework for Training Multi-Speaker TTS Models from Dark Data

This paper presents TTSOps, a fully automated closed-loop framework for constructing multi-speaker text-to-speech (TTS) systems from noisy, uncurated web-scale speech data, often referred to as ``dark data,'' such as online videos. Conventional TTS training pipelines require well-curated corpora with high acoustic quality and accurate text-speech alignment, which severely limits scalability, speaker diversity, and real-world applicability. While recent studies have proposed acoustic-quality-based data selection techniques, they often overlook two critical aspects: (1) the inherent robustness of modern TTS models to noise, and (2) the potential contribution of perceptually low-quality yet informative samples. To address these issues, TTSOps introduces a data-centric training pipeline that integrates three core components: (1) automated data collection from dark data sources, (2) utterance-level dynamic selection of data cleansing methods based on training data quality, and (3) evaluation-in-the-loop data selection using automatically predicted mean opinion scores (MOS) to estimate each utterance's impact on model performance. Furthermore, TTSOps jointly optimizes the corpus and the TTS model in a closed-loop framework by dynamically adapting both data selection and data cleansing processes to the characteristics of the target TTS model. Extensive experiments on Japanese YouTube data demonstrate that TTSOps outperforms conventional acoustic-quality-based baselines in both the naturalness and speaker diversity of synthesized speech.

==> chapter3/tab/fs2/normal_table_Uncleansed.tex <==
\multirow{1}{*}{$58500$}
  &Unselected & $1157 / 2719 (42.6\%)$ \\ \midrule
\multirow{3}{*}{$5128$}
  &Acoustic-quality & $1572 / 2719 (57.8\%)$ \\
  &Ours-Utt & $\mathbf{1764 / 2719 (64.9\%)}$ \\
  &Ours-Spk & $1274 / 2719 (46.9\%)$ \\ \midrule
\multirow{3}{*}{$12172$}
  &Acoustic-quality & $1786 / 2719 (65.7\%)$ \\
  &Ours-Utt & $\mathbf{2114 / 2719 (77.7\%)}$ \\
  &Ours-Spk & $1321 / 2719 (48.6\%)$ \\ \midrule
\multirow{3}{*}{$20390$}
  &Acoustic-quality & $1661 / 2719 (61.1\%)$ \\
  &Ours-Utt & $\mathbf{1989 / 2719 (73.2\%)}$ \\
  &Ours-Spk & $1712 / 2719 (63.0\%)$ \\ \midrule
\multirow{3}{*}{$31038$}
  &Acoustic-quality & $1748 / 2719 (64.3\%)$ \\
  &Ours-Utt & $\mathbf{1955 / 2719 (71.9\%)}$ \\
  &Ours-Spk & $1347 / 2719 (49.5\%)$ 


==> chapter3/tab/glow/normal_table_Uncleansed.tex <==
\multirow{1}{*}{$58500$}
  &Unselected & $0 / 2719 (0.0\%)$ \\ \midrule
\multirow{3}{*}{$5128$}
  &Acoustic-quality & $2068 / 2719 (76.1\%)$ \\
  &Ours-Utt & $\mathbf{2305 / 2719 (84.8\%)}$ \\
  &Ours-Spk & $1735 / 2719 (63.8\%)$ \\ \midrule
\multirow{3}{*}{$12172$}
  &Acoustic-quality & $706 / 2719 (26.0\%)$ \\
  &Ours-Utt & $\mathbf{1510 / 2719 (55.5\%)}$ \\
  &Ours-Spk & $798 / 2719 (29.3\%)$ \\ \midrule
\multirow{3}{*}{$20390$}
  &Acoustic-quality & $90 / 2719 (3.3\%)$ \\
  &Ours-Utt & $\mathbf{305 / 2719 (11.2\%)}$ \\
  &Ours-Spk & $297 / 2719 (10.9\%)$ \\ \midrule
\multirow{3}{*}{$31038$}
  &Acoustic-quality & $19 / 2719 (0.7\%)$ \\
  &Ours-Utt & $\mathbf{29 / 2719 (1.1\%)}$ \\
  &Ours-Spk & $25 / 2719 (0.9\%)$ 

==> chapter4/img/pseudoMOSaq.tex <==
\newcommand{\swsinglepseudomos}[5]{
    \begin{subfigure}{1.0\linewidth}
    \includegraphics[width=1.0\linewidth]{chapter4/img/#1/switching_pseudo_mos_#2.pdf}
    \vspace{#4}
    \caption{#3}
    \vspace{#5}
    \end{subfigure}
}

\begin{figure}[t]
  \centering
  
  \swsinglepseudomos{fs2}{aq}{FastSpeech~2}{-13pt}{5pt}
  \swsinglepseudomos{glow}{ours}{GlowTTS}{-45pt}{10pt}
  
  \caption{
    Cumulative histograms of pseudo MOS. 
    Y-axis value indicates number of speakers with higher score than x-axis value.
    The shaded area corresponds to high-quality speakers.
  }
  \label{fig:swpseudoMOSaq}
\end{figure}    



==> chapter4/img/pseudoMOSours.tex <==
\begin{figure}[t]
  \centering
  
  \swsinglepseudomos{fs2}{ours}{FastSpeech~2}{-13pt}{5pt}
  \swsinglepseudomos{glow}{ours}{GlowTTS}{-45pt}{10pt}
  
  \caption{
    Cumulative histograms of pseudo MOS. 
    Y-axis value indicates number of speakers with higher score than x-axis value.
    The shaded area corresponds to high-quality speakers.
  }
  \label{fig:swpseudoMOSaq}
\end{figure}    



==> chapter4/img/switching.tex <==
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.48\linewidth} % 幅を調整
    \centering
    \includegraphics[width=\linewidth]{chapter4/img/fig/switch1.pdf}
    \caption{For data where Method B results in the highest improvement in quality, Method B is selected and applied to enhance the dataset.}
    \label{fig:switch1}
\end{subfigure}
\hfill % 図の間にスペースを挿入
\begin{subfigure}[b]{0.48\linewidth}
    \centering
    \includegraphics[width=\linewidth]{chapter4/img/fig/switch2.pdf}
    \caption{For data where Method C results in the highest improvement in quality, Method C is selected and applied to enhance the dataset.}
    \label{fig:switch2}
\end{subfigure}
\caption{A proposed data cleansing method that enhances the overall dataset quality by dynamically switching between multiple data cleansing methods for each data point. The method evaluates the quality after applying each candidate preprocessing procedure and adopts the one that achieves the highest quality.}
\label{fig:4:switching}
\end{figure}

==> chapter4/tab/fs2/switching_table_aq.tex <==
\multirow{4}{*}{$5128$}
  &Uncleansed & $1572 / 2719 (57.8\%)$ & $469 / 555 (84.5\%)$ & $1103 / 2164 (51.0\%)$\\
\multirow{4}{*}{$12172$}
  &Uncleansed & $1786 / 2719 (65.7\%)$ & $745 / 912 (81.7\%)$ & $1041 / 1807 (57.6\%)$\\
  &Demucs & $2177 / 2719 (80.1\%)$ & $1008 / 1138 (88.6\%)$ & $1169 / 1581 (73.9\%)$\\
  &Miipher & $2224 / 2719 (81.8\%)$ & $1490 / 1681 (88.6\%)$ & $734 / 1038 (70.7\%)$\\
  &Switching & $\mathbf{2413 / 2719 (88.7\%)}$ & $\mathbf{1533 / 1624 (94.4\%)}$ & $\mathbf{880 / 1095 (80.4\%)}$\\ \midrule
\multirow{4}{*}{$20390$}
  &Uncleansed & $1661 / 2719 (61.1\%)$ & $990 / 1313 (75.4\%)$ & $671 / 1406 (47.7\%)$\\
  &Demucs & $2155 / 2719 (79.3\%)$ & $1322 / 1541 (85.8\%)$ & $\mathbf{833 / 1178 (70.7\%)}$\\
  &Miipher & $\mathbf{2223 / 2719 (81.8\%)}$ & $\mathbf{1799 / 2074 (86.7\%)}$ & $424 / 645 (65.7\%)$\\
  &Switching & $2182 / 2719 (80.3\%)$ & $1706 / 2021 (84.4\%)$ & $476 / 698 (68.2\%)$\\ \midrule
\multirow{4}{*}{$31038$}
  &Uncleansed & $1748 / 2719 (64.3\%)$ & $1231 / 1737 (70.9\%)$ & $517 / 982 (52.6\%)$\\
  &Demucs & $1958 / 2719 (72.0\%)$ & $1564 / 1975 (79.2\%)$ & $394 / 744 (53.0\%)$\\
  &Miipher & $\mathbf{2103 / 2719 (77.3\%)}$ & $\mathbf{1911 / 2351 (81.3\%)}$ & $192 / 368 (52.2\%)$\\
  &Switching & $2078 / 2719 (76.4\%)$ & $1877 / 2351 (79.8\%)$ & $\mathbf{201 / 368 (54.6\%)}$


==> chapter4/tab/fs2/switching_table_ours.tex <==
\multirow{4}{*}{$5128$}
  &Uncleansed & $1764 / 2719 (64.9\%)$ & $538 / 559 (96.2\%)$ & $1226 / 2160 (56.8\%)$\\
\multirow{4}{*}{$12172$}
  &Uncleansed & $2114 / 2719 (77.7\%)$ & $828 / 876 (94.5\%)$ & $1286 / 1843 (69.8\%)$\\
  &Demucs & $2320 / 2719 (85.3\%)$ & $935 / 958 (97.6\%)$ & $1385 / 1761 (78.6\%)$\\
  &Miipher & $2437 / 2719 (89.6\%)$ & $\mathbf{1202 / 1211 (99.3\%)}$ & $1235 / 1508 (81.9\%)$\\
  &Switching & $\mathbf{2524 / 2719 (92.8\%)}$ & $1264 / 1277 (99.0\%)$ & $\mathbf{1260 / 1442 (87.4\%)}$\\ \midrule
\multirow{4}{*}{$20390$}
  &Uncleansed & $1989 / 2719 (73.2\%)$ & $1076 / 1167 (92.2\%)$ & $913 / 1552 (58.8\%)$\\
  &Demucs & $2205 / 2719 (81.1\%)$ & $1238 / 1316 (94.1\%)$ & $967 / 1403 (68.9\%)$\\
  &Miipher & $2318 / 2719 (85.3\%)$ & $\mathbf{1523 / 1551 (98.2\%)}$ & $795 / 1168 (68.1\%)$\\
  &Switching & $\mathbf{2473 / 2719 (91.0\%)}$ & $1576 / 1636 (96.3\%)$ & $\mathbf{897 / 1083 (82.8\%)}$\\ \midrule
\multirow{4}{*}{$31038$}
  &Uncleansed & $1955 / 2719 (71.9\%)$ & $1392 / 1610 (86.5\%)$ & $563 / 1109 (50.8\%)$\\
  &Demucs & $2241 / 2719 (82.4\%)$ & $1545 / 1693 (91.3\%)$ & $696 / 1026 (67.8\%)$\\
  &Miipher & $2204 / 2719 (81.1\%)$ & $1772 / 1869 (94.8\%)$ & $432 / 850 (50.8\%)$\\
  &Switching & $\mathbf{2516 / 2719 (92.5\%)}$ & $\mathbf{1849 / 1927 (96.0\%)}$ & $\mathbf{667 / 792 (84.2\%)}$


==> chapter4/tab/glow/switching_table_aq.tex <==
\multirow{4}{*}{$0$}
  &Uncleansed & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
\multirow{4}{*}{$0$}
  &Uncleansed & $\mathbf{0 / 2719 (0.0\%)}$ & - & $\mathbf{0 / 2719 (0.0\%)}$\\
  &Demucs & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Miipher & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Switching & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\ \midrule
\multirow{4}{*}{$0$}
  &Uncleansed & $\mathbf{0 / 2719 (0.0\%)}$ & - & $\mathbf{0 / 2719 (0.0\%)}$\\
  &Demucs & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Miipher & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Switching & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\ \midrule
\multirow{4}{*}{$0$}
  &Uncleansed & $\mathbf{0 / 2719 (0.0\%)}$ & - & $\mathbf{0 / 2719 (0.0\%)}$\\
  &Demucs & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Miipher & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Switching & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$


==> chapter4/tab/glow/switching_table_ours.tex <==
\multirow{4}{*}{$0$}
  &Uncleansed & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
\multirow{4}{*}{$0$}
  &Uncleansed & $\mathbf{0 / 2719 (0.0\%)}$ & - & $\mathbf{0 / 2719 (0.0\%)}$\\
  &Demucs & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Miipher & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Switching & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\ \midrule
\multirow{4}{*}{$0$}
  &Uncleansed & $\mathbf{0 / 2719 (0.0\%)}$ & - & $\mathbf{0 / 2719 (0.0\%)}$\\
  &Demucs & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Miipher & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Switching & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\ \midrule
\multirow{4}{*}{$0$}
  &Uncleansed & $\mathbf{0 / 2719 (0.0\%)}$ & - & $\mathbf{0 / 2719 (0.0\%)}$\\
  &Demucs & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Miipher & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$\\
  &Switching & $0 / 2719 (0.0\%)$ & - & $0 / 2719 (0.0\%)$


==> img/fig1.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=0.8\linewidth]{img/fig/figure1.pdf} 
    \caption{ 
      Distributions in speaker space for multi-speaker TTS corpus~\cite{takamichi2019jvs} and dark data~(e.g., data from YouTube~\cite{takamichi2021jtubespeech}).
      Compared with speakers in the massive dark data, speakers in TTS corpus are very limited and localized.}
    \label{fig:spk_dist}
\end{figure}

==> img/old_fig1/figure1.tex <==
\begin{figure}[t]
  \centering
    \includegraphics[width=0.8\linewidth]{img/fig/figure1.pdf} 
    \caption{ 
      Distributions in speaker space for multi-speaker TTS corpus~\cite{takamichi2019jvs} and dark data~(e.g., data from YouTube~\cite{takamichi2021jtubespeech}).
      Compared with speakers in the massive dark data, speakers in TTS corpus are very limited and localized.}
    \label{fig:spk_dist}
\end\begin{figure}[t]
  \centering
    \includegraphics[width=0.8\linewidth]{img/fig/figure1.pdf} 
    \caption{ 
      Distributions in speaker space for multi-speaker TTS corpus~\cite{takamichi2019jvs} and dark data~(e.g., data from YouTube~\cite{takamichi2021jtubespeech}).
      Compared with speakers in the massive dark data, speakers in TTS corpus are very limited and localized.}
    \label{fig:spk_dist}
\end{figure}
